Risk-averse optimization of total rewards in Markovian models using deviation measures

This paper addresses objectives tailored to the risk-averse optimization of accumulated rewards in Markov decision processes (MDPs). The studied objectives require maximizing the expected value of the accumulated rewards minus a penalty factor times a deviation measure of the resulting distribution of rewards. Using the variance in this penalty mechanism leads to the variance-penalized expectation (VPE) for which it is known that optimal schedulers have to minimize future expected rewards when a high amount of rewards has been accumulated. This behavior is undesirable as risk-averse behavior should keep the probability of particularly low outcomes low, but not discourage the accumulation of additional rewards on already good executions. The paper investigates the semi-variance, which only takes outcomes below the expected value into account, the mean absolute deviation (MAD), and the semi-MAD as alternative deviation measures. Furthermore, a penalty mechanism that penalizes outcomes below a fixed threshold is studied. For all of these objectives, the properties of optimal schedulers are specified and in particular the question whether these objectives overcome the problem observed for the VPE is answered. Further, the resulting algorithmic problems on MDPs and Markov chains are investigated.

==> sections/experiments.tex <==


\section{Experiments}

\todo[inline]{Brief overview of implementations:

- Gurobi-based for MADPE

- By adding a PRISM-module for the threshold-based penalty.

What machine was used for the experiments? Where is the implementation available?}

To give a proof of concept for applying penalized expectation measures in practice we run a bunch of experiments relying on the PRISM Modelchecker \cite{ChenForejt2013AModelChecker} for the variant of threshold-based penalty.


\subsection{Threshold-based penalty}

For the following diagrams we utilized the Asynchronous Leader Election Protocol by Itai and Rodeh \cite{IR90}. There are MDP models written in the PRISM input language available on the PRISM website where there are $N=3 \dots 10$ processors in a ring that are looking for a leader. The MDPs come with non-negative rewards defined to be either $0$ or $1$.

Now, for each PRISM model $N=3 \dots 8$ we added a single module which implements the reward counter until reaching the threshold and we added a new reward definition based on the counter of rewards in the original model as well. We used $r=\frac{5}{2}$ in our examples as the factor determining the penalty below the threshold. The threshold $t$ itself has been used as input variable, so that we can see for which $t$ PRISM can calculate the maximum expected reward in a reasonable time.

\todo[inline]{One figure with some of the plots. Do we want to include a table with the data?}

\input{sections/experiments/diagram_m3_total_time_in_t}

\input{sections/experiments/diagram_m4_total_time_in_t}

\input{sections/experiments/diagram_m5_total_time_in_t}

\input{sections/experiments/diagram_m6_total_time_in_t}

\input{sections/experiments/diagram_m7_total_time_in_t}

\input{sections/experiments/diagram_m8_total_time_in_t}

The first, yet not surprising observation of our experiments is that the size of the constructed model is linear in $t$.
The more relevant observation is that the PRISM model checker takes linear time in $t$ for finding the maximum expected value of accumulated rewards until reaching a goal state. One could also say that time consumption is linear in the number of states of the constructed model. However at this spoint, there is of cource no conclusion that this holds for all possible models. In the following chart we put all single measures together and display PRISM's total time consuption depending on the number of states of the constructed MDP. We connect those data point that belong to the same value of $N$.

\input{sections/experiments/diagram_all_total_time_in_states}

The diagram shows that for our models the time consumption can roughly estimated linearly in the number of states of the unfolded MDP.
However every value $N=3\dots 8$ seems to have its own specific ratio of time consumption per number of states.
The MDP for $N=8$ is much greater when taking about the number of states compared to the $N=3$ MDP.
In consequence we are more limited when choosing $t$ for $N=8$.

All measures were done on a machine running Windows 10 Pro 22H2, having installed an Intel Core i9-9900K and 32GB RAM.

\subsection{MADPE}

As a proof of concept for solving for an MADPE-optimal scheduler, we used the same Asynchronous Leader Election Protocol models as for the variant of threshold-based penalty. 
Additionally we used PRISM's case studies model of the shared coin protocol of the randomised consensus algorithm of Aspnes and Herlihy \cite{AH90}.
We implemented a toolchain action as follows. First we run PRISM to give us a model representation with all single states, their transitions, rewards and the maximal expected total reward from each state. Second we run a python script which constructs all the constraints as described before to obtain a linearly constrained program with a quadratic objective. The script uses Gurobi \cite{gurobi} to then solve the optimization problem.
We could solve the resulting optimization problems for $N=3\dots6$. With $N=7$ computation took longer than one hour.
The following diagram shows the total time, excluding the step of PRISM building the model, for running the toolchain mapped to the number of reachable states each model has, according to PRISMs output.


\input{sections/experiments/diagram_madpe.tex}
